Counter-Samples: A Stateless Strategy to Neutralize Black Box Adversarial Attacks

Our paper presents a novel defence against black box attacks, where attackers use the victim model as an oracle to craft their adversarial examples. Unlike traditional preprocessing defences that rely on sanitizing input samples, our stateless strategy counters the attack process itself. For every query we evaluate a counter-sample instead, where the counter-sample is the original sample optimized against the attacker's objective. By countering every black box query with a targeted white box optimization, our strategy effectively introduces an asymmetry to the game to the defender's advantage. This defence not only effectively misleads the attacker's search for an adversarial example, it also preserves the model's accuracy on legitimate inputs and is generic to multiple types of attacks. We demonstrate that our approach is remarkably effective against state-of-the-art black box attacks and outperforms existing defences for both the CIFAR-10 and ImageNet datasets. Additionally, we also show that the proposed defence is robust against strong adversaries as well.

==> ImageNet_Baselines.tex <==
\begin{table}[H]
\caption{Imagenet baselines tables. In this table we shows the same AFR for ImageNet dataset}
\resizebox{\textwidth}{!}{%
\begin{tabular}{llllllllllllllllllllll}
          \\ \cline{9-20} 
 &  &  &  &  &  &  & \multicolumn{1}{l|}{} & \multicolumn{1}{c|}{Method}     & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Clean \\ Perf.\end{tabular}} & \multicolumn{1}{c|}{NES}            & \multicolumn{1}{c|}{ZS}             & \multicolumn{1}{c|}{Bandit}         & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Sign\\ Hunter\end{tabular}} & \multicolumn{1}{c|}{ECO}          & \multicolumn{1}{c|}{SimBA}          & \multicolumn{1}{c|}{Sqaure}         & \multicolumn{1}{c|}{SignOPT}        & \multicolumn{1}{c|}{HSJ}            & \multicolumn{1}{c|}{GeoD}           \\ \cline{9-20} 
 &  &  &  &  &  &  & \multicolumn{1}{l|}{} & \multicolumn{1}{c|}{Clean}      & \multicolumn{1}{c|}{0.78}                                                   & \multicolumn{1}{c|}{0.07}           & \multicolumn{1}{c|}{0.125}          & \multicolumn{1}{c|}{0.01}           & \multicolumn{1}{c|}{0}                                                     & \multicolumn{1}{c|}{0}            & \multicolumn{1}{c|}{0.2375}         & \multicolumn{1}{c|}{0}              & \multicolumn{1}{c|}{0.162}          & \multicolumn{1}{c|}{0.6}            & \multicolumn{1}{c|}{0.112}          \\ \cline{9-20} 
 &  &  &  &  &  &  & \multicolumn{1}{l|}{} & \multicolumn{1}{c|}{AS}         & \multicolumn{1}{c|}{0.688}                                                  & \multicolumn{1}{c|}{0.069}          & \multicolumn{1}{c|}{0.477}          & \multicolumn{1}{c|}{0}              & \multicolumn{1}{c|}{0.002}                                                 & \multicolumn{1}{c|}{0}            & \multicolumn{1}{c|}{0.43}           & \multicolumn{1}{c|}{0}              & \multicolumn{1}{c|}{0.834}          & \multicolumn{1}{c|}{0.68}           & \multicolumn{1}{c|}{0.057}          \\ \cline{9-20} 
 &  &  &  &  &  &  & \multicolumn{1}{l|}{} & \multicolumn{1}{c|}{BS}         & \multicolumn{1}{c|}{0.662}                                                  & \multicolumn{1}{c|}{0.132}          & \multicolumn{1}{c|}{0.405}          & \multicolumn{1}{c|}{0.073}          & \multicolumn{1}{c|}{0.002}                                                 & \multicolumn{1}{c|}{0.003}        & \multicolumn{1}{c|}{0.176}          & \multicolumn{1}{c|}{0}              & \multicolumn{1}{c|}{0.903}          & \multicolumn{1}{c|}{0.75}           & \multicolumn{1}{c|}{0.646}          \\ \cline{9-20} 
 &  &  &  &  &  &  & \multicolumn{1}{l|}{} & \multicolumn{1}{c|}{JPEG}       & \multicolumn{1}{c|}{0.75}                                                   & \multicolumn{1}{c|}{0.139}          & \multicolumn{1}{c|}{0.5}            & \multicolumn{1}{c|}{0.037}          & \multicolumn{1}{c|}{0.004}                                                 & \multicolumn{1}{c|}{0}            & \multicolumn{1}{c|}{0.215}          & \multicolumn{1}{c|}{0}              & \multicolumn{1}{c|}{0.925}          & \multicolumn{1}{c|}{0.788}          & \multicolumn{1}{c|}{0.573}          \\ \cline{9-20} 
 &  &  &  &  &  &  & \multicolumn{1}{l|}{} & \multicolumn{1}{c|}{FS}         & \multicolumn{1}{c|}{0.76}                                                   & \multicolumn{1}{c|}{0.075}          & \multicolumn{1}{c|}{0.485}          & \multicolumn{1}{c|}{0}              & \multicolumn{1}{c|}{0.004}                                                 & \multicolumn{1}{c|}{0}            & \multicolumn{1}{c|}{0.2375}         & \multicolumn{1}{c|}{0}              & \multicolumn{1}{c|}{0.926}          & \multicolumn{1}{c|}{0.772}          & \multicolumn{1}{c|}{0.499}          \\ \cline{9-20} 
 &  &  &  &  &  &  & \multicolumn{1}{l|}{} & \multicolumn{1}{c|}{gaussian}   & \multicolumn{1}{c|}{0.75}                                                   & \multicolumn{1}{c|}{0.075}          & \multicolumn{1}{c|}{0.691}          & \multicolumn{1}{c|}{0.05}           & \multicolumn{1}{c|}{0.39}                                                  & \multicolumn{1}{c|}{0.383}        & \multicolumn{1}{c|}{0.87}           & \multicolumn{1}{c|}{0.131}          & \multicolumn{1}{c|}{0.952}          & \multicolumn{1}{c|}{0.756}          & \multicolumn{1}{c|}{0.68}           \\ \cline{9-20} 
 &  &  &  &  &  &  & \multicolumn{1}{l|}{} & \multicolumn{1}{c|}{RND}        & \multicolumn{1}{c|}{0.726}                                                  & \multicolumn{1}{c|}{0.11}           & \multicolumn{1}{c|}{0.535}          & \multicolumn{1}{c|}{0.075}          & \multicolumn{1}{c|}{0.447}                                                 & \multicolumn{1}{c|}{0.577}        & \multicolumn{1}{c|}{0.838}          & \multicolumn{1}{c|}{0.241}          & \multicolumn{1}{c|}{\textbf{0.956}} & \multicolumn{1}{c|}{0.756}          & \multicolumn{1}{c|}{0.667}          \\ \cline{9-20} 
 &  &  &  &  &  &  & \multicolumn{1}{l|}{} & \multicolumn{1}{c|}{Ours k =1}  & \multicolumn{1}{c|}{0.758}                                                  & \multicolumn{1}{c|}{0.56}           & \multicolumn{1}{c|}{0.752}          & \multicolumn{1}{c|}{\textbf{0.468}} & \multicolumn{1}{c|}{0.706}                                                 & \multicolumn{1}{c|}{0.763}        & \multicolumn{1}{c|}{\textbf{0.873}} & \multicolumn{1}{c|}{0.475}          & \multicolumn{1}{c|}{0.955}          & \multicolumn{1}{c|}{0.746}          & \multicolumn{1}{c|}{0.677}          \\ \cline{9-20} 
 &  &  &  &  &  &  & \multicolumn{1}{l|}{} & \multicolumn{1}{c|}{Ours k =10} & \multicolumn{1}{c|}{0.758}                                                  & \multicolumn{1}{c|}{\textbf{0.658}} & \multicolumn{1}{c|}{\textbf{0.851}} & \multicolumn{1}{c|}{\textbf{0.468}} & \multicolumn{1}{c|}{\textbf{0.761}}                                        & \multicolumn{1}{c|}{\textbf{0.8}} & \multicolumn{1}{c|}{\textbf{0.873}} & \multicolumn{1}{c|}{\textbf{0.519}} & \multicolumn{1}{c|}{0.955}          & \multicolumn{1}{c|}{\textbf{0.794}} & \multicolumn{1}{c|}{\textbf{0.696}} \\ \cline{9-20} 
\end{tabular}%
}
\end{table}

==> M_adaptive_queries.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table}[]
\centering
\caption{The query counts of an adaptive adversary employing the averaging strategy against our defence, RND and SND.}
\label{tab:M_adaptive}
\resizebox{\textwidth}{!}{%
\begin{tabular}{ccccccccccc}
& \multicolumn{1}{c|}{}                    & \multicolumn{3}{c|}{\textit{RND}}                                           & \multicolumn{3}{c|}{\textit{SND}}                                & \multicolumn{3}{c|}{\cellcolor[HTML]{EFEFEF}\textit{Ours k= 10}}                                                            \\ \hline
\multicolumn{1}{c|}{}                           & \multicolumn{1}{c|}{Attack}              & M = 1                & M = 5                & \multicolumn{1}{c|}{M = 10}   & M = 1                & M = 5                & \multicolumn{1}{c|}{M = 10}   & \cellcolor[HTML]{EFEFEF}M = 1    & \cellcolor[HTML]{EFEFEF}M = 5    & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}M = 10}   \\ \hline
\multicolumn{1}{c|}{}                           & \multicolumn{1}{c|}{\textit{Bandit}}     & 506.35               & 1132.38              & \multicolumn{1}{c|}{3775.33}  & 188.06               & 404.19               & \multicolumn{1}{c|}{1364.56}  & \cellcolor[HTML]{EFEFEF}273.92   & \cellcolor[HTML]{EFEFEF}3107.5   & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}2543.44}  \\
\multicolumn{1}{c|}{}                           & \multicolumn{1}{c|}{\textit{NES}}        & 589.36               & 1145.82              & \multicolumn{1}{c|}{5723.01}  & 247.65               & 1770.51              & \multicolumn{1}{c|}{5900.92}  & \cellcolor[HTML]{EFEFEF}923.54   & \cellcolor[HTML]{EFEFEF}667.57   & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}7568.21}  \\
\multicolumn{1}{c|}{}                           & \multicolumn{1}{c|}{\textit{ECO}}        & 710.56               & 2254.68              & \multicolumn{1}{c|}{4867.27}  & 507.31               & 5560.68              & \multicolumn{1}{c|}{7272.18}  & \cellcolor[HTML]{EFEFEF}548.05   & \cellcolor[HTML]{EFEFEF}3387.44  & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}14377.66} \\
\multicolumn{1}{c|}{}                           & \multicolumn{1}{c|}{\textit{SignHunter}} & 274.01               & 916.79               & \multicolumn{1}{c|}{2053.87}  & 399.28               & 949.95               & \multicolumn{1}{c|}{2220.04}  & \cellcolor[HTML]{EFEFEF}459.81   & \cellcolor[HTML]{EFEFEF}3429.19  & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}5590.48}  \\
\multicolumn{1}{c|}{}                           & \multicolumn{1}{c|}{\textit{SimBA}}      & 874.6                & 3104.79              & \multicolumn{1}{c|}{5126.08}  & 1236.07              & 3566.93              & \multicolumn{1}{c|}{10783.25} & \cellcolor[HTML]{EFEFEF}1675.23  & \cellcolor[HTML]{EFEFEF}1826.35  & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}3360.42}  \\
\multicolumn{1}{c|}{}                           & \multicolumn{1}{c|}{\textit{Square}}     & 288.57               & 322.4                & \multicolumn{1}{c|}{1336.98}  & 162.23               & 349.31               & \multicolumn{1}{c|}{753.12}   & \cellcolor[HTML]{EFEFEF}112.86   & \cellcolor[HTML]{EFEFEF}528.25   & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}1345.4}   \\
\multicolumn{1}{c|}{\multirow{-7}{*}{\rotatebox{90}{CIFAR-10}}} & \multicolumn{1}{c|}{\textit{ZS}}         & 709.07               & 3019.85              & \multicolumn{1}{c|}{7836.38}  & 474.54               & 2558.4               & \multicolumn{1}{c|}{5100.4}   & \cellcolor[HTML]{EFEFEF}964.221  & \cellcolor[HTML]{EFEFEF}3370.95  & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}6121.04}  \\ \hline
\multicolumn{1}{c|}{}                           & \multicolumn{1}{c|}{\textit{Bandit}}     & 796.068              & 2994.02              & \multicolumn{1}{c|}{7458.41}  & 600.56               & 2438.65              & \multicolumn{1}{c|}{3509.924} & \cellcolor[HTML]{EFEFEF}481.142  & \cellcolor[HTML]{EFEFEF}1249.9   & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}1248.28}  \\
\multicolumn{1}{c|}{}                           & \multicolumn{1}{c|}{\textit{NES}}        & 2945.48              & 15275.41             & \multicolumn{1}{c|}{24870.7}  & 2668.54              & 13633.21             & \multicolumn{1}{c|}{25221.6}  & \cellcolor[HTML]{EFEFEF}2536.518 & \cellcolor[HTML]{EFEFEF}13742.86 & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}26670.48} \\
\multicolumn{1}{c|}{}                           & \multicolumn{1}{c|}{\textit{ECO}}        & 809.398              & 2094.74              & \multicolumn{1}{c|}{3172.46}  & 777.656              & 3164.52              & \multicolumn{1}{c|}{5718.25}  & \cellcolor[HTML]{EFEFEF}510.784  & \cellcolor[HTML]{EFEFEF}4099.61  & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}3709.66}  \\
\multicolumn{1}{c|}{}                           & \multicolumn{1}{c|}{\textit{SignHunter}} & 377.565              & 4197.22              & \multicolumn{1}{c|}{3453.83}  & 302.282              & 899.7                & \multicolumn{1}{c|}{1770.66}  & \cellcolor[HTML]{EFEFEF}170.158  & \cellcolor[HTML]{EFEFEF}238.57   & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}879.1}    \\
\multicolumn{1}{c|}{}                           & \multicolumn{1}{c|}{\textit{SimBA}}      & 373.75               & 2555.56              & \multicolumn{1}{c|}{6962.25}  & 418.31               & 989.18               & \multicolumn{1}{c|}{5461.36}  & \cellcolor[HTML]{EFEFEF}251.193  & \cellcolor[HTML]{EFEFEF}1264.37  & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}3570.95}  \\
\multicolumn{1}{c|}{}                           & \multicolumn{1}{c|}{\textit{Square}}     & 186.27               & 1546.91              & \multicolumn{1}{c|}{791}      & 315.78               & 619.18               & \multicolumn{1}{c|}{1115.01}  & \cellcolor[HTML]{EFEFEF}55.626   & \cellcolor[HTML]{EFEFEF}59.33    & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}583.97}   \\
\multicolumn{1}{c|}{\multirow{-7}{*}{\rotatebox{90}{ImageNet}}} & \multicolumn{1}{c|}{\textit{ZS}}         & 2529.6               & 14593.84             & \multicolumn{1}{c|}{20399.51} & 2514.67              & 8910                 & \multicolumn{1}{c|}{16246.81} & \cellcolor[HTML]{EFEFEF}1535.345 & \cellcolor[HTML]{EFEFEF}5338     & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}12898.88} \\ \hline                           
\end{tabular}%
}
\end{table}

==> baselines_queries.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table}[]
\centering
\caption{The queries count results of all the attacks against our defence and each of the
baselines}
\label{tab:baselines_queries}
\resizebox{\textwidth}{!}{%
\begin{tabular}{cccccccccccc}
\multicolumn{1}{c|}{}                            & \multicolumn{1}{c|}{\textit{Method}}                    & \multicolumn{1}{c|}{\textit{NES}}                     & \multicolumn{1}{c|}{\textit{ZS}}                      & \multicolumn{1}{c|}{\textit{Bandit}}                 & \multicolumn{1}{c|}{\textit{SignHunter}}             & \multicolumn{1}{c|}{\textit{ECO}}                    & \multicolumn{1}{c|}{\textit{SimBA}}                  & \multicolumn{1}{c|}{\textit{Sqaure}}                & \multicolumn{1}{c|}{\textit{SignOPT}}                 & \multicolumn{1}{c|}{\textit{HSJ}}                     & \multicolumn{1}{c|}{\textit{GeoD}}                   \\ \hline
\multicolumn{1}{c|}{}                            & \multicolumn{1}{c|}{\textit{No Defence}}                & \multicolumn{1}{c|}{166.793}                          & \multicolumn{1}{c|}{231.652}                          & \multicolumn{1}{c|}{108.293}                         & \multicolumn{1}{c|}{136.26}                          & \multicolumn{1}{c|}{158.195}                         & \multicolumn{1}{c|}{2834.33}                         & \multicolumn{1}{c|}{59.934}                         & \multicolumn{1}{c|}{1793.83}                          & \multicolumn{1}{c|}{2251.16}                          & \multicolumn{1}{c|}{1081.4}                          \\
\multicolumn{1}{c|}{}                            & \multicolumn{1}{c|}{AS}                                 & \multicolumn{1}{c|}{224.117}                          & \multicolumn{1}{c|}{248.38}                           & \multicolumn{1}{c|}{1046.739}                        & \multicolumn{1}{c|}{100.03}                          & \multicolumn{1}{c|}{90.55}                           & \multicolumn{1}{c|}{3425.76}                         & \multicolumn{1}{c|}{44.01}                          & \multicolumn{1}{c|}{2551.97}                          & \multicolumn{1}{c|}{2886.459}                         & \multicolumn{1}{c|}{568.93}                          \\
\multicolumn{1}{c|}{}                            & \multicolumn{1}{c|}{BS}                                 & \multicolumn{1}{c|}{187.12}                           & \multicolumn{1}{c|}{299.566}                          & \multicolumn{1}{c|}{2054.534}                        & \multicolumn{1}{c|}{75.337}                          & \multicolumn{1}{c|}{98.903}                          & \multicolumn{1}{c|}{2136.39}                         & \multicolumn{1}{c|}{41.021}                         & \multicolumn{1}{c|}{729.941}                          & \multicolumn{1}{c|}{994.784}                          & \multicolumn{1}{c|}{798.515}                         \\
\multicolumn{1}{c|}{}                            & \multicolumn{1}{c|}{JPEG}                               & \multicolumn{1}{c|}{211.997}                          & \multicolumn{1}{c|}{231.351}                          & \multicolumn{1}{c|}{2317.975}                        & \multicolumn{1}{c|}{81.914}                          & \multicolumn{1}{c|}{179.086}                         & \multicolumn{1}{c|}{1510.58}                         & \multicolumn{1}{c|}{48.357}                         & \multicolumn{1}{c|}{925.715}                          & \multicolumn{1}{c|}{1328.12}                          & \multicolumn{1}{c|}{1319.361}                        \\
\multicolumn{1}{c|}{}                            & \multicolumn{1}{c|}{FS}                                 & \multicolumn{1}{c|}{170.987}                          & \multicolumn{1}{c|}{208.9075}                         & \multicolumn{1}{c|}{302}                             & \multicolumn{1}{c|}{138.612}                         & \multicolumn{1}{c|}{161.937}                         & \multicolumn{1}{c|}{2134.64}                         & \multicolumn{1}{c|}{59.048}                         & \multicolumn{1}{c|}{1357.997}                         & \multicolumn{1}{c|}{1236.478}                         & \multicolumn{1}{c|}{1419.755}                        \\
\multicolumn{1}{c|}{}                            & \multicolumn{1}{c|}{SND}                                & \multicolumn{1}{c|}{245.022}                          & \multicolumn{1}{c|}{336.3}                            & \multicolumn{1}{c|}{209.489}                         & \multicolumn{1}{c|}{477.294}                         & \multicolumn{1}{c|}{906.972}                         & \multicolumn{1}{c|}{1236.07}                         & \multicolumn{1}{c|}{241.023}                        & \multicolumn{1}{c|}{727.009}                          & \multicolumn{1}{c|}{1280.04}                          & \multicolumn{1}{c|}{795.992}                         \\
\multicolumn{1}{c|}{}                            & \multicolumn{1}{c|}{RND}                                & \multicolumn{1}{c|}{463.758}                          & \multicolumn{1}{c|}{638.751}                          & \multicolumn{1}{c|}{299.839}                         & \multicolumn{1}{c|}{504.353}                         & \multicolumn{1}{c|}{852.219}                         & \multicolumn{1}{c|}{874.6}                           & \multicolumn{1}{c|}{317.677}                        & \multicolumn{1}{c|}{672.169}                          & \multicolumn{1}{c|}{1366.701}                         & \multicolumn{1}{c|}{809.354}                         \\
\multicolumn{1}{c|}{}                            & \multicolumn{1}{c|}{AT}                                 & \multicolumn{1}{c|}{842.59}                           & \multicolumn{1}{c|}{739.633}                          & \multicolumn{1}{c|}{3441.82}                         & \multicolumn{1}{c|}{1161.06}                         & \multicolumn{1}{c|}{1238.03}                         & \multicolumn{1}{c|}{3964.73}                         & \multicolumn{1}{c|}{1377.33}                        & \multicolumn{1}{c|}{592.62}                           & \multicolumn{1}{c|}{2409.1}                           & \multicolumn{1}{c|}{1251.78}                         \\
\multicolumn{1}{c|}{}                            & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}Ours k =1}  & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}930.57}   & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}1081.61}  & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}306.015} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}296.583} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}563.608} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}2124.71} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}116.71} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}849.189}  & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}1325.17}  & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}834.909} \\
\multicolumn{1}{c|}{\multirow{-10}{*}{\rotatebox{90}{CIFAR-10}}} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}Ours k =10} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}801.481}  & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}964.221}  & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}386.6}   & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}289.572} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}627.7}   & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}1675.23} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}121.39} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}1356.23}  & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}1412.144} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}749.559} \\ \hline
\multicolumn{1}{c|}{}                            & \multicolumn{1}{c|}{\textit{No Defence}}                & \multicolumn{1}{c|}{2598.229}                         & \multicolumn{1}{c|}{1528.74}                          & \multicolumn{1}{c|}{683.734}                         & \multicolumn{1}{c|}{557.12}                          & \multicolumn{1}{c|}{301.7}                           & \multicolumn{1}{c|}{4845}                            & \multicolumn{1}{c|}{122.7}                          & \multicolumn{1}{c|}{6431.11}                          & \multicolumn{1}{c|}{3202.5}                           & \multicolumn{1}{c|}{1219.25}                         \\
\multicolumn{1}{c|}{}                            & \multicolumn{1}{c|}{AS}                                 & \multicolumn{1}{c|}{2165.358}                         & \multicolumn{1}{c|}{838.823}                          & \multicolumn{1}{c|}{508.125}                         & \multicolumn{1}{c|}{389.126}                         & \multicolumn{1}{c|}{246.325}                         & \multicolumn{1}{c|}{4293.146}                        & \multicolumn{1}{c|}{138.755}                        & \multicolumn{1}{c|}{2917.596}                         & \multicolumn{1}{c|}{2028.782}                         & \multicolumn{1}{c|}{1232.194}                        \\
\multicolumn{1}{c|}{}                            & \multicolumn{1}{c|}{BS}                                 & \multicolumn{1}{c|}{3125.491}                         & \multicolumn{1}{c|}{909.87}                           & \multicolumn{1}{c|}{1401.54}                         & \multicolumn{1}{c|}{376.775}                         & \multicolumn{1}{c|}{260.921}                         & \multicolumn{1}{c|}{4103.81}                         & \multicolumn{1}{c|}{148.377}                        & \multicolumn{1}{c|}{1035}                             & \multicolumn{1}{c|}{1660.705}                         & \multicolumn{1}{c|}{662.947}                         \\
\multicolumn{1}{c|}{}                            & \multicolumn{1}{c|}{JPEG}                               & \multicolumn{1}{c|}{2866.632}                         & \multicolumn{1}{c|}{1104.65}                          & \multicolumn{1}{c|}{638.092}                         & \multicolumn{1}{c|}{462.928}                         & \multicolumn{1}{c|}{298.293}                         & \multicolumn{1}{c|}{3049.758}                        & \multicolumn{1}{c|}{134.597}                        & \multicolumn{1}{c|}{1392.428}                         & \multicolumn{1}{c|}{1084.5}                           & \multicolumn{1}{c|}{1300.523}                        \\
\multicolumn{1}{c|}{}                            & \multicolumn{1}{c|}{FS}                                 & \multicolumn{1}{c|}{2549.175}                         & \multicolumn{1}{c|}{1037.251}                         & \multicolumn{1}{c|}{574.35}                          & \multicolumn{1}{c|}{616.68}                          & \multicolumn{1}{c|}{354.694}                         & \multicolumn{1}{c|}{4801.9}                          & \multicolumn{1}{c|}{159.208}                        & \multicolumn{1}{c|}{1292.8214}                        & \multicolumn{1}{c|}{1511.77}                          & \multicolumn{1}{c|}{1457.537}                        \\
\multicolumn{1}{c|}{}                            & \multicolumn{1}{c|}{SND}                                & \multicolumn{1}{c|}{2776.369}                         & \multicolumn{1}{c|}{1304.436}                         & \multicolumn{1}{c|}{801.24}                          & \multicolumn{1}{c|}{302.282}                         & \multicolumn{1}{c|}{777.656}                         & \multicolumn{1}{c|}{418}                             & \multicolumn{1}{c|}{275.924}                        & \multicolumn{1}{c|}{480.388}                          & \multicolumn{1}{c|}{1481.57}                          & \multicolumn{1}{c|}{411.31}                          \\
\multicolumn{1}{c|}{}                            & \multicolumn{1}{c|}{RND}                                & \multicolumn{1}{c|}{2743.474}                         & \multicolumn{1}{c|}{2633.068}                         & \multicolumn{1}{c|}{796.068}                         & \multicolumn{1}{c|}{377.565}                         & \multicolumn{1}{c|}{809.398}                         & \multicolumn{1}{c|}{373.75}                          & \multicolumn{1}{c|}{235.819}                        & \multicolumn{1}{c|}{454.218}                          & \multicolumn{1}{c|}{1481.57}                          & \multicolumn{1}{c|}{418.214}                         \\
\multicolumn{1}{c|}{}                            & \multicolumn{1}{c|}{AT}                                 & \multicolumn{1}{c|}{2927.33}                          & \multicolumn{1}{c|}{1376.51}                          & \multicolumn{1}{c|}{1046.882}                        & \multicolumn{1}{c|}{1426.07}                         & \multicolumn{1}{c|}{1327.82}                         & \multicolumn{1}{c|}{5219.83}                         & \multicolumn{1}{c|}{1131.74}                        & \multicolumn{1}{c|}{2615.38}                          & \multicolumn{1}{c|}{299.4}                            & \multicolumn{1}{c|}{1584.53}                         \\
\multicolumn{1}{c|}{}                            & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}Ours k =1}  & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}3249.238} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}1955.043} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}152.25}  & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}231.368} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}539.428} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}403}     & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}48.61}  & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}437.176}  & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}1905.75}  & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}464.53}  \\
\multicolumn{1}{c|}{\multirow{-10}{*}{\rotatebox{90}{ImageNet}}} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}Ours k =10} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}2536.518} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}1535.345} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}481.142} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}170.158} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}510.784} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}251}     & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}55.626} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}1530.352} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}1391.125} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}391.185} \\ \hline
                             
\end{tabular}%
}
\end{table}

==> l2_AFR.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\centering
\caption{The Attack Failure Rate (AFR) of all attacks against our defence method.}
\label{tab:l2_AFR}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lllllllllll}
    
      &                           &                            &                           &                            &                           &                           &                                &                             &                           &                            \\
\multicolumn{1}{c}{}          & \multicolumn{1}{c}{}      & \multicolumn{1}{c}{}       & \multicolumn{1}{c}{}      & \multicolumn{1}{c}{}       & \multicolumn{1}{c}{}      & \multicolumn{1}{c}{}      & \multicolumn{1}{c}{}           & \multicolumn{1}{c}{}        & \multicolumn{1}{c}{}      & \multicolumn{1}{c}{}       \\
\multicolumn{1}{c|}{Dataset}  & \multicolumn{1}{c}{ZS}    & \multicolumn{1}{c}{Bandit} & \multicolumn{1}{c}{NES}   & \multicolumn{1}{c}{Square} & \multicolumn{1}{c}{SimBA} & \multicolumn{1}{c}{ECO}   & \multicolumn{1}{c}{SignHunter} & \multicolumn{1}{c}{SignOPT} & \multicolumn{1}{c}{HSJ}   & \multicolumn{1}{c|}{GeoD}  \\ \hline
\multicolumn{1}{c|}{CIFAR-10} & \multicolumn{1}{c}{0.758} & \multicolumn{1}{c}{0.517}  & \multicolumn{1}{c}{0.727} & \multicolumn{1}{c}{0.482}  & \multicolumn{1}{c}{0.839} & \multicolumn{1}{c}{0.775} & \multicolumn{1}{c}{0.574}      & \multicolumn{1}{c}{0.848}   & \multicolumn{1}{c}{0.545} & \multicolumn{1}{c|}{0.6}   \\ \hline
\multicolumn{1}{c|}{ImageNet} & \multicolumn{1}{c}{0.86}  & \multicolumn{1}{c}{0.81}   & \multicolumn{1}{c}{0.8}   & \multicolumn{1}{c}{0.796}  & \multicolumn{1}{c}{0.848} & \multicolumn{1}{c}{0.86}  & \multicolumn{1}{c}{0.797}      & \multicolumn{1}{c}{0.949}   & \multicolumn{1}{c}{0.909} & \multicolumn{1}{c|}{0.886} \\ \hline
      &                           &                            &                           &                            &                           &                           &                                &                             &                           &                          
\end{tabular}%
}
\end{table}

==> l2_queries.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\centering
\caption{The query counts of the $\ell_{2}$ norm attacks against our defence method.}
\label{tab:l2_queries}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lllllllllll}
                                        &                                      &                                  &                                    \\
\multicolumn{1}{c|}{Dataset}  & \multicolumn{1}{c}{\textit{ZS}} & \multicolumn{1}{c}{\textit{Bandit}} & \multicolumn{1}{c}{\textit{NES}} & \multicolumn{1}{c}{\textit{Square}} & \multicolumn{1}{c}{\textit{SimBA}} & \multicolumn{1}{c}{\textit{ECO}} & \multicolumn{1}{c}{\textit{SignHunter}} & \multicolumn{1}{c}{\textit{SignOPT}} & \multicolumn{1}{c}{\textit{HSJ}} & \multicolumn{1}{c|}{\textit{GeoD}} \\ \hline
\multicolumn{1}{c|}{CIFAR-10} & \multicolumn{1}{c}{160}         & \multicolumn{1}{c}{429.357}         & \multicolumn{1}{c}{1128.91}     & \multicolumn{1}{c}{243.8}           & \multicolumn{1}{c}{384.28}         & \multicolumn{1}{c}{627.7}        & \multicolumn{1}{c}{252.29}              & \multicolumn{1}{c}{1356.23}          & \multicolumn{1}{c}{698.75}       & \multicolumn{1}{c|}{892.02}        \\ \hline
\multicolumn{1}{c|}{ImageNet} & \multicolumn{1}{c}{851.09}      & \multicolumn{1}{c}{102.6}           & \multicolumn{1}{c}{3198.93}      & \multicolumn{1}{c}{209.875}         & \multicolumn{1}{c}{467.33}         & \multicolumn{1}{c}{660.272}      & \multicolumn{1}{c}{175.87}              & \multicolumn{1}{c}{579.75}           & \multicolumn{1}{c}{2765.571}     & \multicolumn{1}{c|}{173.222}       \\ \hline
\multicolumn{1}{c}{}          & \multicolumn{1}{c}{}            & \multicolumn{1}{c}{}                & \multicolumn{1}{c}{}             & \multicolumn{1}{c}{}                & \multicolumn{1}{c}{}               & \multicolumn{1}{c}{}             & \multicolumn{1}{c}{}                    & \multicolumn{1}{c}{}                 & \multicolumn{1}{c}{}             & \multicolumn{1}{c}{}               \\

\end{tabular}%
}
\end{table}

==> step_size_queries.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table}[]
\centering
\caption{The query counts results of an adaptive adversary utilizing different step sizes in each iteration. The step size is determined by the default one multiply by the step size factor.}
\label{tab:step_size_queries}
\resizebox{\textwidth}{!}{%
\begin{tabular}{ccccc|ccc|ccc|ccc|}
                                                &                                             & \multicolumn{3}{c|}{ZoSignSGD}                                                                      & \multicolumn{3}{c|}{Bandit}                                                                        & \multicolumn{3}{c|}{NES}                                                                            & \multicolumn{3}{c|}{SimBA}                                                                          \\ \hline
\multicolumn{1}{c|}{}                           & Defence                                     & x1                               & x2                              & x10                            & x1                              & x2                              & x10                            & x1                               & x2                              & x10                            & x1                              & x2                              & x10                             \\ \hline
\multicolumn{1}{c|}{}                           & \textit{AS}                                 & 248.38                           & 212.51                          & 661.94                         & 1046.739                        & 617.7                           & 211.97                         & 224.117                          & 152.67                          & 229.59                         & 3425.76                         & 1900.41                         & 605.63                          \\
\multicolumn{1}{c|}{}                           & \textit{BS}                                 & 299.566                          & 368                             & 417.43                         & 2054.534                        & 1452.56                         & 288.79                         & 187.12                           & 297.6                           & 635.27                         & 2136.39                         & 1183.69                         & 358.75                          \\
\multicolumn{1}{c|}{}                           & \textit{JPEG}                               & 231.351                          & 581.18                          & 681.8                          & 2317.975                        & 2714.37                         & 742.5                          & 211.997                          & 441.54                          & 413.67                         & 1510.58                         & 1269.19                         & 803.31                          \\
\multicolumn{1}{c|}{}                           & \textit{FS}                                 & 208.9075                         & 259.59                          & 197.54                         & 302                             & 673.322                         & 55.03                          & 170.987                          & 186                             & 748.83                         & 2134.64                         & 1197.39                         & 356.53                          \\
\multicolumn{1}{c|}{}                           & \textit{SND}                                & 336.3                            & 472.8                           & 450.38                         & 209.489                         & 1737.55                         & 568.86                         & 245.022                          & 421.02                          & 334.26                         & 1236.07                         & 1234.46                         & 733.58                          \\
\multicolumn{1}{c|}{}                           & \textit{RND}                                & 638.751                          & 423.66                          & 778.029                        & 299.839                         & 1261.94                         & 626.944                        & 463.758                          & 438.89                          & 745.38                         & 874.6                           & 874.62                          & 1077.17                         \\
\multicolumn{1}{c|}{\multirow{-7}{*}{\rotatebox{90}{CIFAR10}}}  & \cellcolor[HTML]{EFEFEF}\textit{Ours k =10} & \cellcolor[HTML]{EFEFEF}964.221  & \cellcolor[HTML]{EFEFEF}1335.33 & \cellcolor[HTML]{EFEFEF}703.07 & \cellcolor[HTML]{EFEFEF}386.6   & \cellcolor[HTML]{EFEFEF}1438.27 & \cellcolor[HTML]{EFEFEF}876.35 & \cellcolor[HTML]{EFEFEF}801.481  & \cellcolor[HTML]{EFEFEF}1070.48 & \cellcolor[HTML]{EFEFEF}626.64 & \cellcolor[HTML]{EFEFEF}1675.23 & \cellcolor[HTML]{EFEFEF}1440.3  & \cellcolor[HTML]{EFEFEF}1314.92 \\ \hline
\multicolumn{1}{c|}{}                           & \textit{AS}                                 & 838.823                          & 559.12                          & 779.42                         & 508.125                         & 421.04                          & 408.416                        & 2165.358                         & 1340.3                          & 657.6                          & 4293.146                        & 4242.12                         & 408.41                          \\
\multicolumn{1}{c|}{}                           & \textit{BS}                                 & 909.87                           & 1351.08                         & 768.8                          & 745.761                         & 1162.68                         & 819.92                         & 3125.491                         & 1746.155                        & 1241.84                        & 4166.821                        & 4103.81                         & 819.92                          \\
\multicolumn{1}{c|}{}                           & \textit{JPEG}                               & 1104.65                          & 1528.48                         & 910.27                         & 638.092                         & 713.61                          & 389.684                        & 2866.632                         & 1807.55                         & 703.71                         & 3049.758                        & 3133.16                         & 3133.16                         \\
\multicolumn{1}{c|}{}                           & \textit{FS}                                 & 1037.251                         & 813                             & 625.81                         & 574.35                          & 639.08                          & 543.075                        & 2549.175                         & 1452                            & 814.53                         & 4801.9                          & 4878.11                         & 4878.11                         \\
\multicolumn{1}{c|}{}                           & \textit{SND}                                & 1304.436                         & 1261.21                         & 1338.16                        & 600.56                          & 803.34                          & 441.95                         & 2776.369                         & 1655.97                         & 837.18                         & 420.42                          & 418.14                          & 441.95                          \\
\multicolumn{1}{c|}{}                           & \textit{RND}                                & 2633.068                         & 1612                            & 412.11                         & 796.068                         & 436.18                          & 487.46                         & 2743.474                         & 1842.08                         & 715.62                         & 1328.376                        & 775.75                          & 775.75                          \\
\multicolumn{1}{c|}{\multirow{-7}{*}{\rotatebox{90}{ImageNet}}} & \cellcolor[HTML]{EFEFEF}\textit{Ours k =10} & \cellcolor[HTML]{EFEFEF}1535.345 & \cellcolor[HTML]{EFEFEF}1064.33 & \cellcolor[HTML]{EFEFEF}882.58 & \cellcolor[HTML]{EFEFEF}481.142 & \cellcolor[HTML]{EFEFEF}106.1   & \cellcolor[HTML]{EFEFEF}131.26 & \cellcolor[HTML]{EFEFEF}2536.518 & \cellcolor[HTML]{EFEFEF}1747.24 & \cellcolor[HTML]{EFEFEF}235.63 & \cellcolor[HTML]{EFEFEF}251     & \cellcolor[HTML]{EFEFEF}1336.63 & \cellcolor[HTML]{EFEFEF}1336.72 \\ \hline
\end{tabular}%
}
\end{table}
